Non-Perturbative Effects in Matrix Models and Vacua of Two Dimensional Gravity

The most general large N eigenvalues distribution for the one matrix model is shown to consist of tree-like structures in the complex plane. For the m=2 critical point, such a split solution describes the strong coupling phase of 2d quantum gravity (c=0 non-critical string). It is obtained by taking combinations of complex contours in the matrix integral, and the relative weight of the contours is identified with the non-perturbative theta-parameter that fixes uniquely the solution of the string equation (Painleve I). This allows to recover by instanton methods results on the non-perturbative effects obtained by the Isomonodromic Deformation Method, and to construct for each theta-vacuum the observables (the loop correlation functions) which satisfy the loop equations. The breakdown of analyticity of the large N solution is related to the existence of poles for the loop operators.

==> 9212106.2 <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%   FIGURES: extract the following  postscript file and print it (3 pages)   %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%% END OF TEX FILE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%!
%%Title: /tmp/xfig-export025366
%%Creator: fig2dev
%%CreationDate: Tue Dec 15 10:32:00 1992
%%For: david@wasa (Francois David,774 16A,28111,)
%%BoundingBox: 242 188 594 522
%%Pages: 1
%%EndComments
/$F2psDict 6400 dict def
$F2psDict begin
$F2psDict /mtrx matrix put
/l {lineto} bind def
/m {moveto} bind def
/s {stroke} bind def
/n {newpath} bind def
/gs {gsave} bind def
/gr {grestore} bind def
/clp {closepath} bind def
/graycol {dup dup currentrgbcolor 4 -2 roll mul 4 -2 roll mul
4 -2 roll mul setrgbcolor} bind def
/col-1 {} def
/col0 {0 0 0 setrgbcolor} bind def
/col1 {0 0 1 setrgbcolor} bind def
/col2 {0 1 0 setrgbcolor} bind def
/col3 {0 1 1 setrgbcolor} bind def
/col4 {1 0 0 setrgbcolor} bind def
/col5 {1 0 1 setrgbcolor} bind def
/col6 {1 1 0 setrgbcolor} bind def
/col7 {1 1 1 setrgbcolor} bind def
	end
	/$F2psBegin {$F2psDict begin /$F2psEnteredState save def} def
	/$F2psEnd {$F2psEnteredState restore end} def
	%%EndProlog

$F2psBegin
0 setlinecap 0 setlinejoin
-112.0 751.0 translate 0.900 -0.900 scale
0.500 setlinewidth
% Polyline
n 472 208 m 472 580 l gs col-1 s gr
% Polyline
n 659 279 m 286 509 l gs col-1 s gr
% Polyline
n 286 279 m 659 509 l gs col-1 s gr
2.000 setlinewidth
% Polyline
n 444 344 m 462 344 l  458 362 l gs col-1 s gr
% Polyline
n 440 441 m 458 441 l  451 423 l gs col-1 s gr
% Polyline
n 515 401 m 526 387 l  537 401 l gs col-1 s gr
% Interpolated spline
n 587 208 m
	523.734 284.628 495.007 316.892 472 337 curveto
	463.196 344.526 440.910 360.910 429 365 curveto
	401.492 375.735 361.095 381.112 268 387 curveto
gs col-1 s gr
% Interpolated spline
n 587 580 m
	523.734 503.372 495.007 471.108 472 451 curveto
	463.196 443.474 440.910 427.090 429 423 curveto
	401.492 412.265 361.095 406.888 268 401 curveto
gs col-1 s gr
% Interpolated spline
n 598 215 m
	553.112 294.278 536.055 330.127 530 358 curveto
	526.108 374.183 526.019 410.210 530 426 curveto
	536.079 453.755 553.136 488.708 598 566 curveto
gs col-1 s gr
/Times-Italic findfont 20.00 scalefont setfont
419 334 m
gs 1 -1 scale (C) col-1 show gr
/Times-Italic findfont 20.00 scalefont setfont
419 479 m
gs 1 -1 scale (C) col-1 show gr
/Times-Italic findfont 20.00 scalefont setfont
564 399 m
gs 1 -1 scale (C) col-1 show gr
/Times-Roman findfont 12.00 scalefont setfont
434 339 m
gs 1 -1 scale (+) col-1 show gr
/Times-Roman findfont 12.00 scalefont setfont
434 484 m
gs 1 -1 scale (-) col-1 show gr
/Times-Italic findfont 12.00 scalefont setfont
579 404 m
gs 1 -1 scale (i) col-1 show gr
showpage
$F2psEnd
/$F2psDict 6400 dict def
$F2psDict begin
$F2psDict /mtrx matrix put
/l {lineto} bind def
/m {moveto} bind def
/s {stroke} bind def
/n {newpath} bind def
/gs {gsave} bind def
/gr {grestore} bind def
/clp {closepath} bind def
/graycol {dup dup currentrgbcolor 4 -2 roll mul 4 -2 roll mul
4 -2 roll mul setrgbcolor} bind def
/col-1 {} def
/col0 {0 0 0 setrgbcolor} bind def
/col1 {0 0 1 setrgbcolor} bind def
/col2 {0 1 0 setrgbcolor} bind def
/col3 {0 1 1 setrgbcolor} bind def
/col4 {1 0 0 setrgbcolor} bind def
/col5 {1 0 1 setrgbcolor} bind def
/col6 {1 1 0 setrgbcolor} bind def
/col7 {1 1 1 setrgbcolor} bind def
 /DrawSplineSection {
	/y3 exch def
	/x3 exch def
	/y2 exch def
	/x2 exch def
	/y1 exch def
	/x1 exch def
	/xa x1 x2 x1 sub 0.666667 mul add def
	/ya y1 y2 y1 sub 0.666667 mul add def
	/xb x3 x2 x3 sub 0.666667 mul add def
	/yb y3 y2 y3 sub 0.666667 mul add def
	x1 y1 lineto
	xa ya xb yb x3 y3 curveto
	} def

	end
	/$F2psBegin {$F2psDict begin /$F2psEnteredState save def} def
	/$F2psEnd {$F2psEnteredState restore end} def
	%%EndProlog

$F2psBegin
0 setlinecap 0 setlinejoin
88.0 625.5 translate 0.900 -0.900 scale
2.000 setlinewidth
% Polyline
n 119 139 m 339 139 l gs col-1 s gr
0.500 setlinewidth
% Polyline
n 224 174 m 239 179 l  224 184 l gs col-1 s gr
2.000 setlinewidth
% Polyline
n 269 329 m 409 329 l gs col-1 s gr
% Polyline
n 199 329 m 74 329 l  79 329 l gs col-1 s gr
0.500 setlinewidth
% Polyline
n 234 364 m 244 369 l  234 374 l gs col-1 s gr
% Closed spline
n 99.000 139.000 m
	99.000 139.000 99.000 159.000 139.000 169.000 DrawSplineSection
	139.000 169.000 179.000 179.000 229.000 179.000 DrawSplineSection
	229.000 179.000 279.000 179.000 319.000 169.000 DrawSplineSection
	319.000 169.000 359.000 159.000 359.000 139.000 DrawSplineSection
	359.000 139.000 359.000 119.000 319.000 109.000 DrawSplineSection
	319.000 109.000 279.000 99.000 229.000 99.000 DrawSplineSection
	229.000 99.000 179.000 99.000 139.000 109.000 DrawSplineSection
	139.000 109.000 99.000 119.000 99.000 139.000 DrawSplineSection closepath gs
col-1 s gr
% Open spline
n 159.000 329.000 m 164.000 341.500 l
	164.000 341.500 169.000 354.000 194.000 361.500 DrawSplineSection
	194.000 361.500 219.000 369.000 239.000 369.000 DrawSplineSection
	239.000 369.000 259.000 369.000 284.000 361.500 DrawSplineSection
	284.000 361.500 309.000 354.000 314.000 341.500 DrawSplineSection
	319.000 329.000 l gs col-1 s gr
	[4.000000] 0 setdash
% Open spline
n 159.000 324.000 m 164.000 311.500 l
	164.000 311.500 169.000 299.000 194.000 291.500 DrawSplineSection
	194.000 291.500 219.000 284.000 239.000 284.000 DrawSplineSection
	239.000 284.000 259.000 284.000 284.000 291.500 DrawSplineSection
	284.000 291.500 309.000 299.000 314.000 311.500 DrawSplineSection
	319.000 324.000 l gs col-1 s gr
	[] 0 setdash
/Times-Roman findfont 16.00 scalefont setfont
224 219 m
gs 1 -1 scale (\(a\)) col-1 show gr
/Times-Roman findfont 16.00 scalefont setfont
229 409 m
gs 1 -1 scale (\(b\)) col-1 show gr
showpage
$F2psEnd
/$F2psDict 6400 dict def
$F2psDict begin
$F2psDict /mtrx matrix put
/l {lineto} bind def
/m {moveto} bind def
/s {stroke} bind def
/n {newpath} bind def
/gs {gsave} bind def
/gr {grestore} bind def
/clp {closepath} bind def
/graycol {dup dup currentrgbcolor 4 -2 roll mul 4 -2 roll mul
4 -2 roll mul setrgbcolor} bind def
/col-1 {} def
/col0 {0 0 0 setrgbcolor} bind def
/col1 {0 0 1 setrgbcolor} bind def
/col2 {0 1 0 setrgbcolor} bind def
/col3 {0 1 1 setrgbcolor} bind def
/col4 {1 0 0 setrgbcolor} bind def
/col5 {1 0 1 setrgbcolor} bind def
/col6 {1 1 0 setrgbcolor} bind def
/col7 {1 1 1 setrgbcolor} bind def
 /DrawEllipse {
	/endangle exch def
	/startangle exch def
	/yrad exch def
	/xrad exch def
	/y exch def
	/x exch def
	/savematrix mtrx currentmatrix def
	x y translate xrad yrad scale 0 0 1 startangle endangle arc
	savematrix setmatrix
	} def newpath 0 0 0 0 0 1 DrawEllipse stroke

 /DrawSplineSection {
	/y3 exch def
	/x3 exch def
	/y2 exch def
	/x2 exch def
	/y1 exch def
	/x1 exch def
	/xa x1 x2 x1 sub 0.666667 mul add def
	/ya y1 y2 y1 sub 0.666667 mul add def
	/xb x3 x2 x3 sub 0.666667 mul add def
	/yb y3 y2 y3 sub 0.666667 mul add def
	x1 y1 lineto
	xa ya xb yb x3 y3 curveto
	} def

	end
	/$F2psBegin {$F2psDict begin /$F2psEnteredState save def} def
	/$F2psEnd {$F2psEnteredState restore end} def
	%%EndProlog

$F2psBegin
0 setlinecap 0 setlinejoin
34.0 670.5 translate 0.540 -0.540 scale
0.000 setlinewidth
% Polyline
n 299 704 m 329 724 l  354 749 l  374 779 l
 394 814 l  414 859 l  369 874 l  319 879 l  279 879 l
 239 874 l  189 864 l  199 849 l  209 819 l  224 789 l
 234 749 l  269 729 l  clp gs 0.80 setgray fill gr
% Polyline
n 702 375 m 717 355 l  732 335 l  742 315 l
 752 295 l  762 275 l  767 260 l  767 250 l  792 260 l
 817 265 l  842 280 l  867 295 l  882 315 l  902 335 l
 862 360 l  802 375 l  747 380 l  clp gs 0.80 setgray fill gr
/Times-Roman findfont 30.00 scalefont setfont
212 1005 m
gs 1 -1 scale (\(c\)) col-1 show gr
% Polyline
n 799 694 m 829 674 l  854 649 l  874 619 l
 894 584 l  914 539 l  869 524 l  819 519 l  779 519 l
 739 524 l  689 534 l  699 549 l  709 579 l  724 609 l
 734 649 l  769 669 l  clp gs 0.80 setgray fill gr
% Polyline
n 232 15 m 312 10 l  397 15 l  442 30 l
 412 50 l  382 85 l  362 115 l  342 155 l  332 175 l
 327 195 l  332 215 l  342 235 l  352 255 l  367 280 l
 382 300 l  397 320 l  417 340 l  437 360 l  392 380 l
 322 385 l  267 380 l  232 375 l  252 345 l  262 315 l
 272 295 l  272 270 l  267 240 l  262 220 l  257 205 l
 252 195 l  262 175 l  267 155 l  272 125 l  272 105 l
 267 80 l  257 60 l  247 40 l  242 25 l  clp gs 0.80 setgray fill gr
% Polyline
n 702 15 m 717 35 l  732 55 l  742 75 l
 752 95 l  762 115 l  767 130 l  767 140 l  792 130 l
 817 125 l  842 110 l  867 95 l  882 75 l  902 55 l
 862 30 l  802 15 l  747 10 l  clp gs 0.80 setgray fill gr
% Polyline
n 259 484 m 284 524 l  299 554 l  314 589 l
 326 634 l  369 629 l  409 609 l  439 589 l  469 559 l
 493 519 l  440 496 l  373 486 l  314 484 l  clp gs 0.80 setgray fill gr
% Polyline
n 759 914 m 784 874 l  799 844 l  814 809 l
 826 764 l  869 769 l  909 789 l  939 809 l  969 839 l
 993 879 l  940 902 l  873 912 l  814 914 l  clp gs 0.80 setgray fill gr
3.000 setlinewidth
	[10.000000] 0 setdash
% Polyline
n 532 195 m 572 195 l gs col-1 s gr
	[] 0 setdash
% Polyline
n 52 195 m 252 195 l gs col-1 s gr
	[10.000000] 0 setdash
% Polyline
n 14 704 m 79 705 l gs 0.50 setgray fill gr
gs col-1 s gr
	[] 0 setdash
% Polyline
n 572 195 m 712 195 l gs col-1 s gr
1.000 setlinewidth
% Ellipse
n 302 195 2 2 0 360 DrawEllipse gs 1.00 setgray fill gr
gs col-1 s gr
3.000 setlinewidth
	[10.000000] 0 setdash
% Polyline
n 12 195 m 52 195 l gs col-1 s gr
	[] 0 setdash
0.500 setlinewidth
% Open spline
n 252.000 195.000 m 257.000 185.000 l
	257.000 185.000 262.000 175.000 267.000 155.000 DrawSplineSection
	267.000 155.000 272.000 135.000 272.000 115.000 DrawSplineSection
	272.000 115.000 272.000 95.000 262.000 70.000 DrawSplineSection
	262.000 70.000 252.000 45.000 242.000 30.000 DrawSplineSection
	232.000 15.000 l gs col-1 s gr
% Open spline
n 252.000 195.000 m 257.000 205.000 l
	257.000 205.000 262.000 215.000 267.000 235.000 DrawSplineSection
	267.000 235.000 272.000 255.000 272.000 275.000 DrawSplineSection
	272.000 275.000 272.000 295.000 262.000 320.000 DrawSplineSection
	262.000 320.000 252.000 345.000 242.000 360.000 DrawSplineSection
	232.000 375.000 l gs col-1 s gr
% Interpolated spline
n 327 195 m
	329.510 183.351 330.760 178.351 332 175 curveto
	335.586 165.307 346.863 143.853 352 135 curveto
	360.284 120.725 381.463 87.853 392 75 curveto
	400.266 64.917 421.220 42.770 432 35 curveto
	433.598 33.848 436.098 32.598 442 30 curveto
gs col-1 s gr
% Interpolated spline
n 327 195 m
	329.510 206.649 330.760 211.649 332 215 curveto
	335.586 224.693 346.862 246.147 352 255 curveto
	360.284 269.275 381.463 302.147 392 315 curveto
	400.266 325.083 421.220 347.230 432 355 curveto
	433.598 356.152 436.098 357.402 442 360 curveto
gs col-1 s gr
% Open spline
n 767.000 140.000 m 764.500 127.500 l
	764.500 127.500 762.000 115.000 754.500 97.500 DrawSplineSection
	754.500 97.500 747.000 80.000 734.500 60.000 DrawSplineSection
	734.500 60.000 722.000 40.000 712.000 27.500 DrawSplineSection
	702.000 15.000 l gs col-1 s gr
3.000 setlinewidth
	[10.000000] 0 setdash
% Polyline
n 514 694 m 579 693 l gs 0.50 setgray fill gr
gs col-1 s gr
	[] 0 setdash
0.500 setlinewidth
% Open spline
n 767.000 250.000 m 764.500 262.500 l
	764.500 262.500 762.000 275.000 754.500 292.500 DrawSplineSection
	754.500 292.500 747.000 310.000 734.500 330.000 DrawSplineSection
	734.500 330.000 722.000 350.000 712.000 362.500 DrawSplineSection
	702.000 375.000 l gs col-1 s gr
% Open spline
n 767.000 140.000 m 777.000 137.500 l
	777.000 137.500 787.000 135.000 807.000 127.500 DrawSplineSection
	807.000 127.500 827.000 120.000 847.000 107.500 DrawSplineSection
	847.000 107.500 867.000 95.000 884.500 75.000 DrawSplineSection
	902.000 55.000 l gs col-1 s gr
3.000 setlinewidth
% Open spline
n 712.000 195.000 m 727.000 182.500 l
	727.000 182.500 742.000 170.000 754.500 155.000 DrawSplineSection
	767.000 140.000 l gs col-1 s gr
% Open spline
n 712.000 195.000 m 727.000 207.500 l
	727.000 207.500 742.000 220.000 754.500 235.000 DrawSplineSection
	767.000 250.000 l gs col-1 s gr
0.500 setlinewidth
% Interpolated spline
n 302 705 m
	320.923 718.292 328.923 724.292 334 729 curveto
	342.995 737.341 361.684 759.249 369 769 curveto
	374.881 776.838 387.436 796.309 392 805 curveto
	396.956 814.437 402.956 828.687 416 862 curveto
gs col-1 s gr
% Interpolated spline
n 231 748 m
	244.313 739.880 250.063 736.380 254 734 curveto
	259.684 730.565 273.471 722.718 279 719 curveto
	282.556 716.609 287.556 712.859 299 704 curveto
gs col-1 s gr
% Interpolated spline
n 231 748 m
	226.267 770.095 224.017 779.595 222 786 curveto
	217.704 799.644 206.093 831.334 199 844 curveto
	196.868 847.806 193.118 852.806 184 864 curveto
gs col-1 s gr
% Interpolated spline
n 326 634 m
	319.491 610.723 316.491 600.723 314 594 curveto
	310.083 583.430 299.131 559.022 294 549 curveto
	288.572 538.397 279.822 523.397 259 489 curveto
gs col-1 s gr
% Interpolated spline
n 326 634 m
	353.771 632.687 365.771 631.437 374 629 curveto
	385.998 625.446 410.857 611.844 421 605 curveto
	430.673 598.473 451.316 580.885 459 572 curveto
	466.210 563.663 474.710 550.413 493 519 curveto
gs col-1 s gr
% Interpolated spline
n 302 705 m
	320.923 718.292 328.923 724.292 334 729 curveto
	342.995 737.341 361.684 759.249 369 769 curveto
	374.881 776.838 387.436 796.309 392 805 curveto
	396.956 814.437 402.956 828.687 416 862 curveto
gs col-1 s gr
3.000 setlinewidth
% Interpolated spline
n 79 705 m
	109.141 707.496 122.141 708.746 131 710 curveto
	142.042 711.563 168.201 715.717 179 719 curveto
	187.420 721.560 206.410 729.379 214 734 curveto
	217.292 736.004 221.542 739.504 231 748 curveto
gs col-1 s gr
% Interpolated spline
n 299 704 m
	301.496 689.468 302.746 683.218 304 679 curveto
	305.766 673.061 311.253 659.537 314 654 curveto
	315.784 650.402 318.784 645.402 326 634 curveto
gs col-1 s gr
0.500 setlinewidth
% Interpolated spline
n 731 650 m
	744.313 658.120 750.063 661.620 754 664 curveto
	759.684 667.435 773.471 675.282 779 679 curveto
	782.556 681.391 787.556 685.141 799 694 curveto
gs col-1 s gr
% Interpolated spline
n 731 650 m
	726.267 627.905 724.017 618.405 722 612 curveto
	717.704 598.356 706.093 566.666 699 554 curveto
	696.868 550.194 693.118 545.194 684 534 curveto
gs col-1 s gr
% Interpolated spline
n 826 764 m
	819.491 787.277 816.491 797.277 814 804 curveto
	810.083 814.570 799.131 838.978 794 849 curveto
	788.572 859.603 779.822 874.603 759 909 curveto
gs col-1 s gr
% Interpolated spline
n 826 764 m
	853.771 765.313 865.771 766.563 874 769 curveto
	885.998 772.554 910.857 786.156 921 793 curveto
	930.673 799.527 951.316 817.115 959 826 curveto
	966.210 834.337 974.710 847.587 993 879 curveto
gs col-1 s gr
% Interpolated spline
n 802 693 m
	820.923 679.708 828.923 673.708 834 669 curveto
	842.995 660.659 861.684 638.751 869 629 curveto
	874.880 621.162 887.436 601.691 892 593 curveto
	896.956 583.563 902.956 569.313 916 536 curveto
gs col-1 s gr
3.000 setlinewidth
% Interpolated spline
n 579 693 m
	609.141 690.504 622.141 689.254 631 688 curveto
	642.042 686.437 668.201 682.283 679 679 curveto
	687.420 676.440 706.410 668.621 714 664 curveto
	717.292 661.996 721.542 658.496 731 650 curveto
gs col-1 s gr
% Interpolated spline
n 799 694 m
	801.496 708.532 802.746 714.782 804 719 curveto
	805.766 724.939 811.253 738.463 814 744 curveto
	815.784 747.598 818.784 752.598 826 764 curveto
gs col-1 s gr
0.500 setlinewidth
% Open spline
n 767.000 250.000 m 777.000 252.500 l
	777.000 252.500 787.000 255.000 807.000 262.500 DrawSplineSection
	807.000 262.500 827.000 270.000 847.000 282.500 DrawSplineSection
	847.000 282.500 867.000 295.000 884.500 315.000 DrawSplineSection
	902.000 335.000 l gs col-1 s gr
/Times-Roman findfont 30.00 scalefont setfont
712 435 m
gs 1 -1 scale (\(b\)) col-1 show gr
/Times-Roman findfont 30.00 scalefont setfont
212 435 m
gs 1 -1 scale ( \(a\)) col-1 show gr
/Times-Roman findfont 30.00 scalefont setfont
694 1004 m
gs 1 -1 scale (\(d\)) col-1 show gr
showpage
$F2psEnd



